Kyrix-S: Authoring Scalable Scatterplot Visualizations of Big Data

Static scatterplots often suffer from the overdraw problem on big datasets where object overlap causes undesirable visual clutter. The use of zooming in scatterplots can help alleviate this problem. With multiple zoom levels, more screen real estate is available, allowing objects to be placed in a less crowded way. We call this type of visualization scalable scatterplot visualizations, or SSV for short. Despite the potential of SSVs, existing systems and toolkits fall short in supporting the authoring of SSVs due to three limitations. First, many systems have limited scalability, assuming that data fits in the memory of one computer. Second, too much developer work, e.g., using custom code to generate mark layouts or render objects, is required. Third, many systems focus on only a small subset of the SSV design space (e.g. supporting a specific type of visual marks). To address these limitations, we have developed Kyrix-S, a system for easy authoring of SSVs at scale. Kyrix-S derives a declarative grammar that enables specification of a variety of SSVs in a few tens of lines of code, based on an existing survey of scatterplot tasks and designs. The declarative grammar is supported by a distributed layout algorithm which automatically places visual marks onto zoom levels. We store data in a multi-node database and use multi-node spatial indexes to achieve interactive browsing of large SSVs. Extensive experiments show that 1) Kyrix-S enables interactive browsing of SSVs of billions of objects, with response times under 500ms and 2) Kyrix-S achieves 4X-9X reduction in specification compared to a state-of-the-art authoring system.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> src/intro_old.tex <==
%%%%%%%%%%%%%% Introduction %%%%%%%%%%%%%%
\vspace{-.5em}
\ifCLASSOPTIONcompsoc
\IEEEraisesectionheading{\section{Introduction}\label{sec:introduction}}
\else
\section{Introduction}
\label{sec:introduction}
\fi
\vspace{-.5em}

\IEEEPARstart{Z}{oomable} visualizations are an essential component of visual exploratory systems. In this class of visualizations, the user explores one semantic data space via pan or zoom actions (e.g. consider Google Maps), or jumping from one semantic space to another (e.g. jumping from maps to street views). Such paradigm is a perfect example of the visual information seeking mantra\cite{shneiderman1996eyes}: \textit{Overview first, zoom and filter, then details on demand}. 
%By presenting data at different levels of details with positional contexts,

% ------ unresolved ------- 
%\remco{this class is undefined. You need to define what ZSVs are -- don't forget to mention early on that scatterplot falls into this class. Otherwise readers are going to imagine maps.}
%\remco{the first two paragraphs need a little bit of work. I don't think that paragraph 1 is strictly necessary. It can be merged into the second. The reason is that we need to jump as quickly as possible to the definition of ZSVs -- until then the reader wouldn't have context about what's going on.}
% ------ unresolved ------- 

In this paper, we focus on a special type of zoomable visualizations with a single 2D semantic space, which we call \textit{zoomable space visualizations} (ZSV). We assume that the data is stored in a relational database and has two fields $X$ and $Y$ specifying the location of each object. A ZSV thus visualizes objects from such a database using multiple zoom levels that share the same coordinate system (with different scales). One or a group of objects can be rendered as arbitrary shapes such as circles or size-bounded polygons. In a sense, ZSVs are one class of ``generalized scatterplots''\cite{sarikaya2017scatterplots} which visualize 2D scatter data but are not limited to point marks.

ZSVs are especially effective at visualizing large amounts of data (millions to billions of objects), which is our focus. By expanding the 2D plane into multiple zoom levels, more screen resolution becomes available, thus allowing visual marks to be placed in a way that avoids overcrowded displays. We can also use visual aggregates\cite{elmqvist2009hierarchical}(e.g. circles or heatmaps) to show aggregation information of a group of objects.
Figure \ref{fig:teaser} shows a circle-based ZSV created by the system we introduce in this paper, which visualizes one billion comments made by users on \texttt{Reddit.com} from January 2013 to February 2015, where $X$ is the posting time and $Y$ is the length of the comments. Additional examples can be found in Figure \ref{fig:gallery}. 

There has been significant work on building systems/toolkits to aid the creation of ZSVs (e.g. \cite{tao2019kyrix,bederson1994pad++,guo2018efficient,das2012efficient}). These existing systems can be classified into two categories: \textit{specialized ZSV systems} and \textit{general pan/zoom systems}. Specialized ZSV systems (e.g. \cite{guo2018efficient,chen2014visual}) typically have a narrow focus on ZSVs, while general pan/zoom systems such as ZVTM\cite{pietriga2005toolkit} and Kyrix\cite{tao2019kyrix} are more broad, supporting more data types (e.g. temporal and hierarchical) and zoomable visualizations with multiple semantic spaces. 

However, while these systems have been shown to be effective, they can suffer from some drawbacks that limit their ability to support general ZSV authoring at scale. In particular, \textbf{limited scalability} is a common drawback of both types of systems. As often as not, implementations assume all objects reside in the main memory of a computer\cite{wang2015spatial, chen2014visual, mayorga2013splatterplots, liao2017cluster, guo2018efficient,lins2013nanocubes,miranda2017topkube,bederson1994pad++,pietriga2005toolkit}. 
%\remco{all these systems should be mentioned in the categorization above (between specialized ZSVs versus general pan/zoom systems}
%wenbo: there is too many. maybe we should just use examples in categorization?

Another drawback of specialized ZSV systems is \textbf{low expressivity}. Oftentimes systems are coded for a single type of visual mark, e.g., points \cite{das2012efficient, chen2014visual} or heatmaps\cite{perrot2015large,lins2013nanocubes}, and are not extensible to more general scenarios. 

General pan/zoom systems, while being more expressive, generally incur \textbf{too much manual effort} due to their low-level nature. When authoring a ZSV, the developer needs to manually generate the layout of visual marks on zoom levels. In very large datasets, there will be many levels (e.g. Google Maps have 20). Individually specifying the layout of a set of levels is tedious and error-prone. In particular, skewed data can make it challenging for the developer to specify a layout that avoids occlusion and excessive density in the visualization.

%%general-purpose zoomable visualizations\cite{bederson1994pad++,bederson2003jazz,pietriga2005toolkit}, and our contribution is called Kyrix\cite{tao2019kyrix}.

%\subhead{Too much manual effort}. Many general-purpose systems do not assist the developer in generating the layout of visual marks on zoom levels\cite{bederson1994pad++,tao2019kyrix,pietriga2005toolkit}. In very large datasets, there will be many levels (e.g. Google Maps have 20). Individually coding the layout of a set of levels is tedious. Skewed data can make it challenging to avoid occlusion and excessive density. Moreover, these systems are often low-level. The developer needs to specify verbose renderers that convert data to visual marks. 


%Non-overlapping circles represent clusters of comments, with numbers inside indicating the size of the cluster. Through pan or zoom, the user can navigate this multi-scale data space to get either an overview (left) or inspect an area of interest (middle). By hovering over a circle, the user can see the three highest-scored comments and the bounding rectangle of all comments in the cluster. 

%While it is possible to create ZSVs using general pan/zoom systems, the authoring process is in fact problematic.
%First, the developer is required to manually place visual marks on each zoom level, which is a challenging task especially on big skewed datasets where simple strategies (e.g. random sampling) can easily lead to visual clutter in dense regions.  % In fact, layout generation in ZSVs has been researched for more than a decade\cite{dix2002chance,derthick2003constant,wang2015spatial,guo2018efficient,liao2017cluster}. Thus it is impractical to leave this job to the developer who is often not an expert in this area.\sys, on the other hand, automates the layout generation.
%Second, the code/specification is often verbose due to their low-level nature. Visual data mapping (e.g. scaling/aggregating/rendering data) is often developer-defined. Despite high customizability, writing those custom code is error-prone and time-consuming. 
%In contrast, \sys abstract these away by offering a high-level declarative grammar with only a few required parameters. 
%Finally, most of these systems can only handle small data that fits in memory, which is ultimately not scalable. While Kyrix\cite{tao2019kyrix} supports large disk-resident data, it only works with a single-node database which has limited scalability. 

%Numerous specialized ZSV systems exist, but they often suffer from low flexibility and scalability. Many focus on specific types of visual marks, e.g., small-sized dots \cite{das2012efficient, chen2014visual} and heatmap\cite{perrot2015large,lins2013nanocubes}. Many assumes that data fits in the main memory of one computer\cite{wang2015spatial, chen2014visual, mayorga2013splatterplots, liao2017cluster, guo2018efficient} and therefore cannot scale to large data. 

%In addition to ZSVs which feature two meaningful axes and a common coordinate system shared by zoom levels, these systems also generate a wide range of other types of zoomable visualizations such as zoomable treemaps of hierarchical data, semantic zooming to a zoom level with a different coordinate system, etc. 

%\IEEEPARstart{S}{patial} data visualizations such as attraction maps and scatterplots are an essential component of exploratory visualization systems. By visualizing objects on a 2D cartesian plane decorated with visual channels such as axes and background maps, these visualizations provide domain analysts with positional contexts of the underlying data, allowing them to both inspect individual objects and find global patterns that drive important decision making.

%For big and skewed datasets, visualizing every single object inevitably leads to overcrowded displays. To address visual clutter, there has been substantial research~\cite{moritz2019falcon, lins2013nanocubes, liu2013immens, jo2018declarative,heimerl2018visual} on devising aggregated visualizations (e.g. density maps and bar charts). While aggregated visualizations are free of visual clutter, they lack the functionality to query individual objects, which is often crucial in many tasks performed with spatial visualizations\cite{sarikaya2017scatterplots, elmqvist2009hierarchical,park2017atom}. Prior research also studied how to use transparency\cite{fekete2002interactive, kosara2002focus+}, animation\cite{chen2018using} and displacement of objects\cite{waldeck2004mobile, keim1998gridfit, trutschl2003intelligently} to ease the overdraw problem. However, due to limited screen resolution and human perception ability, these approaches have limited scalability.

%On the other hand, zoomable spatial visualizations (ZSV) possess great potential to mitigate visual clutter. By expanding the 2D plane into multiple zoom levels, more screen resolution becomes available, allowing visual marks to be placed in a way that possibly avoids occlusion and excessive density. Interacting with large amounts of individual objects thus becomes feasible. Visual aggregates such as circles or heatmap can also be used to show aggregate statistics of a cluster of objects. 

%This is a scatterplot of 17.3M liquor purchases by retailers in Iowa since 2012, where $x$ and $y$ axes are respectively the unit price (dollars) and quantity (\# of bottles) of purchases. Non-overlapping pies show clusters of purchases grouped by day of the week. By hovering over a pie, the user can see three most recent purchases from the cluster and the boundary of the cluster. 

\begin{figure*}[t]
\centering
\includegraphics[width=1\textwidth]{figs/autodd_teaser.pdf}
\vspace{-2em}
\caption{A ZSV created by \sys and its specification in \sys's declarative grammar. This is a visualization of one billion comments made by users on \texttt{Reddit.com} from Jan 2013 to Feb 2015. X and Y axes are respectively the posting time and length of the comments. Each circle represents a cluster of comments. The number inside each circle is the size of the cluster and also encodes the radius of the circle. As can be seen, the distribution of comments is roughly uniform over time but rather skewed in length. Through pan or zoom, the user can navigate this multi-scale data space to get either an overview (left) or inspect an area of interest (middle). One can hover over a circle to see three highest-scored comments in the cluster, as well as a bounding box showing the boundary of the cluster. \label{fig:teaser}}
\vspace{-1.5em}
\end{figure*}

% , while allowing many tasks typically performed with spatial visualizations such as interaction with individual objects and focused exploration within a neighborhood\cite{sarikaya2017scatterplots}.

%Overview is very useful -- highly-paid players tend to be old. users can zoom in to see more pies   

% For example, Figure \ref{fig:examples}c is a ZSV of NBA basketball games constructed by the system we describe in this paper. The user can see a few exemplary games on the top zoom level, and zoom in to see more games.

% \begin{figure}[t]
% \centering
% \includegraphics[width=0.35\textwidth]{figs/autodd_tvcg_running_example_screenshot2.pdf}
% \vspace{-.5em}
% \caption{A ZSV generated by \sys. This is a scatterplot of 17.3 million liquor purchases by retailers in Iowa since 2012. X and Y axes are respectively the unit price (dollars) and quantity (\# of bottles) of the purchases. Each pie shows a cluster of purchases grouped by day of the week. One can hover over a pie to see a tabular visualization of three most recent purchases, as well as a convex hull showing the boundary of the cluster. \label{fig:runningexamplescreenshot}}
% \vspace{-1.5em}
% \end{figure}

%Despite the utility of ZSVs, programming such visualizations remains a daunting task for application developers, especially when the data is large and skewed. The reasons are multifold. 

%Firstly, tools for creating general zoomable visualizations (e.g. Kyrix\cite{tao2019kyrix}, Pad++\cite{bederson1994pad++}, Jazz\cite{bederson2003jazz} and ZVTM\cite{pietriga2005toolkit}) require the developer to manually place visual marks on each zoom level to manage clutter and occlusion on his/her own. This is a challenging and time-consuming task especially on big and skewed datasets\cite{dix2002chance,wang2015spatial,guo2018efficient}. 
% Arguably, this has been a challenging research topic for more than a decade\cite{dix2002chance,wang2015spatial,guo2018efficient}. Therefore, application developers who are often not experts in this area inevitably experience prolonged development and likely unsatisfying end results. Moreover, the developer also needs to author visual-data mappings (e.g. scaling/aggregating/rendering data) for every zoom level, resulting in verbose specifications. 

%Secondly, many prior ZSV systems/tools focus on only a subset of the ZSV design space, preventing the developer from flexibly making application-specific design choices. For example, much attention has been drawn to specific types of visual marks, e.g., small-sized dots \cite{das2012efficient, chen2014visual} and heatmap\cite{perrot2015large,lins2013nanocubes}. Some works focus on overlap removal\cite{beilschmidt2017linear,chen2014visual} while others center on density limits\cite{das2012efficient,perrot2015large,guo2018efficient}. The narrow focuses make these tools hard to extend to general scenarios, require the developer to constantly switch tools for different application requirements and stymie the creation of customized visualizations. 
% (e.g. visual encodings, degree of overlap, density limits, which objects appear on top). 

%Lastly, big skewed datasets pose significant challenges to the scalability of existing ZSV systems. Many systems\cite{wang2015spatial, chen2014visual, mayorga2013splatterplots, liao2017cluster, guo2018efficient} assume that data fits in the memory of one computer, making them ultimately not scalable. Some systems fetch data in user's viewport on the fly\cite{guo2018efficient,drosou2012disc}, which is not viable on skewed datasets where millions of objects in can be in the viewport at the same time. Some systems precompute\cite{chen2014visual,liao2017cluster, das2012efficient, beilschmidt2017linear} the mark layouts of the ZSV, but the precomputation algorithms are not parallelized and thus cannot scale to large datasets. 

%These limitations of existing systems strongly motivate for an integrated system that supports easy specification of a wide range of design choices of ZSVs, and automate the creation of ZSVs at scale. 

% As shown in Figure \ref{fig:architecture}, \sys employs a simple client-server architecture backed by a multi-node database management system. In the offline indexing phase, the developer writes JSON specifications of ZSVs following the declarative grammar of \sys (Section \ref{sec:grammar}), which is then passed to the layout generator. The layout generator places visual marks on zoom levels, computes relevant aggregation statistics and stores these information into spatially partitioned database tables to cope with big skewed datasets (Section \ref{sec:algorithm}). 

% In the online serving phase, as the user interacts with the ZSV using pan and zoom, the frontend is responsible for rendering the visualization, fetching data dynamically from the data fetcher, which in turn sends queries to the database to fetch data. 

\vspace{.2em}
In this paper, we describe \sys, a system for ZSV authoring at scale which addresses all issues of existing systems. 
Specifically, we store objects in a multi-node parallel database using multi-node spatial indexing. As we show in Section \ref{sec:evaluation}, this allows us to respond to any pan/zoom action in under 500 ms on datasets with billions of objects.

We present a declarative grammar for ZSVs, which \sys implements. To enable rapid authoring, we abstract away low-level details such as rendering of visual marks. The developer can author a complex ZSV in a few tens of lines of JSON. We show that compared to a state-of-the-art system, this is 4--9X reduction in specification on several examples. In addition, we build a gallery of ZSVs to show that our grammar is expressive and that the developer can easily extend it to add his/her own visual marks. 

This grammar is supported by an algorithm that automatically chooses the layout of visual marks at all zoom levels, thereby freeing the developer from writing custom code. As experiments show, this algorithm yields pleasing results according to standard usability metrics and scales well to billions of objects. 


%Our goal is to achieve \textit{rapid authoring}, \textit{expressivity}, \textit{usable ZSVs} and \textit{scalability}. The overall architecture is in Figure \ref{fig:architecture}. We design a high-level declarative grammar that expresses a large space of ZSVs. The developer can author a variety of ZSVs by writing just a few tens of lines of JSON. In an offline indexing phase, a layout generator automates the generation of mark layouts on zoom levels under several usability requirements (e.g. free of clutter, bounded density). To cope with big skewed data, we extend the algorithm to work with a multi-node parallel database. To enable interactive pan/zoom browsing at runtime, the data fetcher utilizes sophisticated database spatial indexes to fetch data efficiently. 

%under a number of usability considerations (e.g. free of clutter and high-quality data abstraction).

% The grammar is designed to be highly extensible for creation of custom visualizations and rapid future extension of the system.

%extend partition the 2D plane of a zoom level in a skew-resilient fashion and process each partition in parallel. 
%To enable interactive browsing of the generated ZSVs, we extend Kyrix\cite{tao2019kyrix}, a recent system for creating general zoomable visualizations.


To summarize, we make the following contributions:
\begin{itemize}
\vspace{-.5em}
    \item An integrated system called Kyrix-S for declarative authoring and rendering of ZSVs at scale.
    \item A concise and expressive declarative grammar for describing ZSVs (Section \ref{sec:grammar}).
    \item A framework for offline database indexing and online serving that enables interactive browsing of large-scale ZSVs with usability guarantees (Section \ref{sec:algorithm}). 
\vspace{-.5em}    
%    scalable distributed algorithm for computing the layout of visual marks on zoom levels that meets various usability requirements, along with a data fetching pipeline that ensures interactive response times on (Section \ref{sec:algorithm}). 
\end{itemize}

%\strike{The rest of the paper is organized as follows. We survey related research in Section \ref{sec:relatedwork}. Section \ref{sec:overview} presents a list of design goals of \sys. Section \ref{sec:grammar} describes \sys's declarative grammar. We describe the backend pipeline of \sys in Sections \ref{sec:sysarch} and \ref{sec:algorithm}, and present implementation details in Section \ref{sec:impl}. Section \ref{sec:evaluation} reports experimental results. We discuss limitations and future work in Section \ref{sec:discussion}. Section \ref{sec:conclusion} concludes the paper.} \remco{not useful}

%We show the expressivity of \sys's declarative grammar by building a gallery of ZSVs (Section \ref{sec:grammar}). We also conduct extensive experiments (Section \ref{sec:evaluation}) demonstrating that 1) \sys's declarative grammar achieves significant reduction in authoring effort compared to general pan/zoom systems; 2) \sys's indexing and serving pipeline scales well to datasets with billions of objects while maintaining interactive response times under 500 ms and 3) mark layouts generated by \sys possess reasonable usability measured in standard metrics. 


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.4\textwidth]{figs/autodd_tvcg_running_example_spec.pdf}
% \vspace{-.5em}
% \caption{\sys specification of the ZSV in Figure \ref{fig:runningexamplescreenshot}. \label{fig:runningexamplespec}}
% \vspace{-1.5em}
% \end{figure}


==> src/response.tex <==
%!TEX root = abbr.tex


\noindent Dear Reviewers,

\vspace{.3em}
Thank you very much for your encouraging comments and thoughtful reviews.  We have done our best to address the comments from the summary reviews and individual reviewers. Detailed responses to your comments are below. 

Note that we have removed ``skewed'' in our title according to a reviewer's suggestion (see our response to \textbf{R3C2}). 

\vspace{3em}


\subhead{\Large Responses to Summary Reviews} 

\vspace{1em}

\subhead{SummaryRC1:} \textit{For the final version of the paper please include a listing of the new elements of the approach in comparison to Kyrix (declarative grammar, back-end performance improvement, etc.)}

\vspace{.25em}
\subhead{Response:} We have added in Section \ref{subsec:related_general} a listing of novel aspects of \sys in comparison to Kyrix. To summarize:
\begin{itemize}
\vspace{-.5em}
    \item \sys provides a high-level grammar for \visnames, which enables much shorter specification than what Kyrix's grammar requires for the same \visname (see Section \ref{subsec:authoringexp} for an empirical comparison);
\vspace{-.5em}
    \item \sys implements a layout generator which frees the developer from deciding the layout of objects on zoom levels. Kyrix does not assist the developer in choosing an object layout, which makes authoring \visnames using Kyrix fairly challenging;
\vspace{-.5em}
    \item  \sys is integrated with a distributed database which scales to billions of objects. In contrast, Kyrix only works with a single-node database which cannot scale to billions of objects. 
\vspace{-.5em}
\end{itemize} 

\vspace{3em}




\subhead{SummaryRC2:} \textit{For the final version of the paper please include a more in depth discussion of what in addition to Kyrix can be done by the enhanced system. This was the main discussion point among the reviewers.}
\vspace{.25em}

\subhead{Response:} The listing we added in Section \ref{subsec:related_general} serves as a good summary of what \sys can do in addition to what Kyrix can do. To further complement this listing, we have also added in Section \ref{subsec:related_grammar} more discussion on the novelty of \sys's declarative grammar (see \textbf{R1C1}) and added in Section \ref{sec:impl} more details on what additional work is involved when implementing \sys's grammar on top of Kyrix's grammar (see \textbf{R3C3}). 

\vspace{1em}




\vspace{1em}
\subhead{\Large Responses to Reviewer \#1} 

\vspace{1em}




\subhead{R1C1:} \textit{...a more important thing is whether users can understand its abstractions and use the new primitives easily. I hope that the authors explain how the proposed grammar make easier for users to explore varied types of SSV than the other prior works. For example, users can just change the visualization type by modifying Marks.Cluster.Mode (e.g., “circle” $\rightarrow$ “heatmap”) instead of implementing a low-level renderer for the visualization type.}

\vspace{.25em}

\subhead{Response:} We have added in Section  \ref{subsec:related_grammar} more clarifications on how our grammar enables easier authoring compared to prior grammars. Specifically, we emphasize that \sys's grammar enables 1) convenient switching of mark representations without having to write custom renderers, 2) authoring of multiple zoom levels altogether as opposed to specifying them individually and 3) concise specification of sampling/aggregation semantics across zoom levels. 


\vspace{3em}



\subhead{R1C2:} \textit{...I wonder what kinds of specification changes make Kyrix-S compute offline indexing? ...I hope that the authors clarify when the offline indexing procedure happens and if it can be an obstacle for exploring SSV design space.}

\vspace{.25em}

\subhead{Response:} \sys will re-compute offline indexing when layout related parameters (e.g. $x$ or $y$ axis) are altered by developer specifications. Currently, to enable quick turnaround when refining an \visname, we allow the developer to direct \sys to compute only a few top zoom levels or use a sample of the data. It is our future work to consider more incremental updates to the data structure upon specification changes. We have added relevant discussions in Section \ref{sec:discussion}. 

% \vspace{3em}




% \subhead{R1C3:} \textit{My concerns are only about the evaluation about authoring efforts...I also think conducting a human-subject study is the best, but it is hard and beyond the expected contribution of 9-page-paper.}

% \vspace{.25em}

% \subhead{Response:} We thank the reviewer for the thoughtful response. As noted, a human-subject study is beyond the scope of the current project. However, as future work we will investigate the use of Kyrix-S in the wild and collect evidence of the usability of the Kyrix-S system and declarative grammar.

\vspace{1em}





\vspace{1em}
\subhead{\Large Responses to Reviewer \#2} 

\vspace{1em}




\subhead{R2C1:} \textit{...and their declarative grammar for producing the visualizations. While this is a functioning specification that solves the design goals, I am missing why the authors selected this form of grammar and not another? To see this seems a bit straight forward and ad hoc - is there anything behind this selection?}

\vspace{.25em}

\subhead{Response:} The high-level structure of the grammar is inspired by the survey of scatterplots by Sarikaya et al.\cite{sarikaya2017scatterplots}. This survey extracted four design variables of scatterplot designs which correspond to the three high-level components in \sys's grammar: \textit{Marks} (mapping to design variables \textit{point encoding} and \textit{point grouping}), \textit{Layout} (mapping to the design variable \textit{point position}) and \textit{Config} (mapping to the design variable \textit{graph amenities}). We have rephrased the first paragraph of Section \ref{subsec:grammarspec} to make this point more clear. 

In Section \ref{subsec:grammarspec}, we have also justified more detailed design choices by connecting them with the design goals listed in Section \ref{sec:overview}. For example, to increase visual expressivity and support inspection of individual objects (\textbf{G2}), we design the \textit{Ranklist} component which visualizes top-k important objects in addition to \textit{Cluster} marks. 

\vspace{3em}




\subhead{R2C2:} \textit{In Section 6.2. the authors describe their efficient clustering algorithm, followed by the multi-node distributed layout algorithm. Again, even though I think the authors made a good selection, I cannot see why they choose this type of strategy, I don't see valid discussions of alternatives and a rationale why a solution was selected.}

\vspace{.25em}

\subhead{Response:} We have revised our writing to include more rationale for our algorithmic choices, as well as discussions on alternatives. More specifically,
\begin{itemize}
\vspace{-.5em}
    \item we have added one paragraph at the beginning of Section \ref{subsec:singlenodealgo} which summarizes the two high-level algorithmic choices of the single-node algorithm, and indicates what the specific design goals they are for;
\vspace{-.5em}
    \item we have revised the writing in Section \ref{subsec:singlenodealgo} to add more intuitions for low-level choices. We originally had a paragraph at the end of Section \ref{subsec:singlenodealgo} to describe how the hierarchical clustering helped us realize some design goals. We have now moved those points to earlier paragraphs in order to justify the algorithm descriptions early on;
\vspace{-.5em}
    \item we have emphasized more at the beginning of Section \ref{subsec:singlenodealgo} that we focus on exact positioning of objects in this paper, and that obvious alternatives would be those considering inexact positioning of objects (e.g. binned aggregation), which is one line of future work we mention in Section \ref{sec:discussion};
\vspace{-.5em}
    \item we have added one paragraph in Section \ref{subsec:multinodealgo} describing the rationale for partitioning the data spatially (as opposed to using other fields). The motivation was to satisfy the overlap and density constraints more easily.
\vspace{-.5em}
\end{itemize}

\vspace{1em}






\vspace{1em}
\subhead{\Large Responses to Reviewer \#3} 

\vspace{1em}




\subhead{R3C1:} \textit{It would be even more impactful if the author could open-source the code...}

\vspace{.25em}

\subhead{Response:} \sys is open source at \url{https://github.com/tracyhenry/kyrix}. We have added this link as a footnote in the introduction. 

\vspace{3em}




\subhead{R3C2:} \textit{The title suggests the paper is focused on the big skewed data. However, I feel it is not reflected much in the content of the paper. ... I suggest that the authors can remove the "skewed" or rephrase a little bit to avoid potential confusion.}

\vspace{.25em}

\subhead{Response:} Thanks for this suggestion. We agree with the reviewer, and have removed the ``skew'' in the title and other places when appropriate. 

%We thank the reviewers for this comment and agree that some uses of skew in the original paper caused confusion. We have removed unnecessary mentions of ``skew'' in places such as the caption of the teaser figure. At the same time, we think it is still relevant to stress the skewness of the data when discussing how it might cause visual clutter and pose algorithmic challenges. The reasons are that (1) skewed datasets are pretty common (in fact all examples in Figures \ref{fig:teaser} and \ref{fig:gallery} have skewed data distributions), and require our backend algorithms (e.g. spatial partitioning) to be skew-resilient;  (2) skewed data distribution can cause significant visual clutter even when the data size is small (e.g. Figure \ref{fig:gallery}c and Figure \ref{fig:gallery}f). 

%We have removed the mentioning of skew in a number of places including the caption of Figure \ref{fig:teaser}. 

% \wenbo{Need to be careful here.}
% \remco{Wenbo, I am wondering if we just remove the word ``skew'' from the title and the text. I think removing the mention of it (or downplaying it) does not change the contribution. In fact, I think the current title sounds like it's limiting the contribution to ``only'' work on skew data... By removing the word ``skew'' you might convey a broader sense of generalizability and therefore adoption and visibility.}

\vspace{3em}





\subhead{R3C3:} \textit{In Section 4, regarding the implementation of the declarative grammar, it is not very clear to me whether it is built from scratch, or it is built upon some existing work (like Kyrix or Vega)... If it is indeed incremental, I want to understand more about how much additional work involved, which helps justify the contribution.}

\vspace{.25em}

\subhead{Response:} As we mention in Section \ref{sec:impl}, we build \sys on top of Kyrix, which means that internally \sys specifications are compiled into low-level Kyrix specifications and that part of Kyrix's frontend rendering is reused. However, since \sys advances Kyrix to support easier and more scalable \visname authoring, we have to extend Kyrix from all angles. Specifically,
\begin{itemize}
\vspace{-.5em}
    \item since \sys supports a distributed database (which Kyrix does not), we have entirely overridden Kyrix's index generator and data fetcher to implement the layout generator using spatial partitioning. 
    We also need to write shell scripts to automate the deployment and maintenance of the distributed database. 
    %These in total amount to roughly 1,500 lines of backend code and 1,000 lines of shell scripts.  
    %As mentioned in Section \ref{subsec:authoringexp}, the implementation of the layout generator alone takes 1,439 lines of code. 
\vspace{-.5em}
    \item since \sys's grammar is new and higher level, we have built a separate compiler to validate developer specifications and translate them into lower-level Kyrix specifications;
\vspace{-.5em}
    \item \sys has a number of mark templates built-in to support easy switching of mark representations. Since Kyrix asks the developer to write custom renderers, we need to write those built-in renderers as part of \sys.
\vspace{-.5em}    
\end{itemize}


\vspace{3em}




\subhead{R3C4:} \textit{On the evaluation side, I feel one important component missing is the demonstration of the usability of the tool. From an end-user perspective, we want to compare this with some "baseline" methods to demonstrate the efficacy of the proposed system..}

\vspace{.25em}

\subhead{Response:} We thank the reviewer for this comment. We agree that the effectiveness of the grammar should be evaluated. In the paper, we use Kyrix as the ``baseline'' and demonstrate the efficiency of the \sys specification in terms of authoring effort (see Section \ref{subsec:authoringexp}). We have made this point more clear in Section \ref{subsec:authoringexp}. 

%We did not perform a human-subject study to measure usability. For our response to such comment, please see our response to R1C3 above.

\vspace{3em}





\subhead{R3C5:} \textit{Minor -- Section 5 has a single paragraph as a section. Since it tells an overview of the framework design, I think it can occur earlier in the paper and merge with other sections (like Section 3).}

\vspace{.25em}

\subhead{Response:} We thank the reviewer for this helpful comment. After a few tries in merging Section \ref{sec:sysarch} into the section before or after, we found that, although short and simple, the section is necessary to establish the overall framework of the Kyrix-S system, and smooth out the flow of text between Sections \ref{sec:grammar} and \ref{sec:algorithm}. As such we have elected to keep the section as it is.

\vspace{1em}






\vspace{1em}
\subhead{\Large Responses to Reviewer \#4} 

\vspace{1em}





\subhead{R4C1:} \textit{The introduction, abstract, and first figure's caption are a little slow to get started and don't quite prime the reader for the (strong) contributions of the paper. I would suggest priming the user that existing systems (Kyrix), task organizations (e.g., scatterplots, clutter reduction), and designs were used to derive a declarative visualization grammar and associated multi-node system to support the grammar. }

\vspace{.25em}

\subhead{Response:} In the revised paper, we have shortened the caption of the teaser figure, the abstract and the introduction to get to our main contributions faster. We have also rephrased relevant text in abstract and the introduction to prime the reader that our main contributions are a declarative grammar for \visnames, as well as a multi-node indexing algorithm and a data fetching pipeline supporting the grammar. 

\vspace{3em}




\subhead{R4C2:} \textit{Table 1 doesn't really add anything over the existing prose.}

\vspace{.25em}

\subhead{Response:} We have removed Table 1. 

\vspace{3em}





\subhead{R4C3:} \textit{Terms like "too much manual effort" could be replaced by more direct terms such as "designer specification"... the former appears as though even visualization viewers struggle with using SSVs in the wild.}

\vspace{.25em}

\subhead{Response:} We have replaced all occurrences of ``too much manual effort'' with ``too much developer work''. 

\vspace{3em}





\subhead{R4C4:} \textit{I might suggest explicitly denoting required and optional attributes in Figure 3 when laying out the grammar, as well as potentially denoting the defaults if omitted (if space allows). }

\vspace{.25em}

\subhead{Response:} We have revised Figure \ref{fig:grammar} to use square brackets to denote optional components. 

\vspace{3em}




\subhead{R4C5:} \textit{Bringing up the importance policy (G3-d) however, it's unclear how this default policy supports identifying outliers (an issue which isn't quite addressed anywhere in the paper).}

\vspace{.25em}

\subhead{Response:} Since our algorithm merges clusters that are within a distance threshold, an outlier would be preserved automatically if it is sufficiently distant from other objects, since it would not be merged into any other cluster. To identify less isolated outliers using the current system, one would need to assign to each object a score (i.e. the importance field) indicating how distant an object is from other objects. Kernel density estimations would be an example of such type of score. It is our future work to automate the identification of outliers. 
We have added relevant discussions in Section \ref{subsec:singlenodealgo}.


%Note that sometimes the application may prefer hiding outliers. As a future work, we plan to make showing/hiding outliers a configurable option to our algorithm.  \wenbo{???}

\vspace{3em}





\subhead{R4C6:} \textit{I was hoping for more of a discussion of how the design decisions that went into the construction of the grammar affected the eventual task support of generated visualizations. }

\vspace{.25em}

\subhead{Response:} We believe this comment is related to the lack of motivation for design decisions mentioned by R2 (see \textbf{R2C1} above). As suggested by R2 and R4, we clarify in Section 4.2 how we designed \sys grammar to support the the tasks already established by Sarikaya et al.\cite{sarikaya2017scatterplots} in their survey of scatterplot visualizations. 

%Please see our response to R2C1 above. To summarize, we did not perform a ``task analysis'' for this paper because we found that the survey by Sarikaya et al.~\cite{sarikaya2017scatterplots} has already explored the space thoroughly. As such, we designed the Kyrix-S grammar to reflect the design space defined by Sarikaya et al. We have rephrased Section \ref{subsec:grammarspec} to make this point clearer.

\vspace{3em}




\subhead{R4C7:} \textit{Section 2.2 (fifth paragraph): "broader design space" is ambiguous here, be a little more specific.}

\vspace{.25em}

\subhead{Response:} We have rephrased it to ``more stringent requirements on the design space'', and refer the readers to Section \ref{sec:overview} for more detailed description of those requirements. 

\vspace{3em}




\subhead{R4C8:} \textit{Footnote 3 should be written in-line or omitted.}

\vspace{.25em}

\subhead{Response:} We have moved it to the main text in Section \ref{subsec:related_general}.

\vspace{3em}





\subhead{R4C9:} \textit{Section 4.2: Clarify what a "rule" is (first instance that this word is used)}

\vspace{.25em}

\subhead{Response:} We have added a footnote to the first occurrence of a ``rule'' to clarify what it means. 

\vspace{3em}




\subhead{R4C10:} \textit{Section 4.2.1: Re-reference the figure where the rules appear}

\vspace{.25em}

\subhead{Response:} We have added a footnote to the first ``rule'' indicating that all following occurrences implicitly refer to rules in Figure \ref{fig:grammar}. 

\vspace{3em}





\subhead{R4C11:} \textit{Section 4.2.1: Why can't "custom" also be used for an aggregation function (rule 14)? I might imagine that an aggregated data point has some custom aggregates defined for it that a defined custom renderer takes advantage of?}

\vspace{.25em}

\subhead{Response:} This is indeed a great point. \sys currently only supports SQL group-by style aggregation using the \textit{Dimension} and \textit{Measure} components. We will consider enabling customization to aggregation in the future. 

\vspace{3em}





\subhead{R4C12:} \textit{Section 4.2.2: "An optional Extent component (Rule 21)..." -- I'm not able to grok this sentence... what does this control?}

\vspace{.25em}

\subhead{Response:} The \textit{Extent} component controls the range of raw $x/y$ values visible on the top zoom level. We have revised the text to be more clear. 

\vspace{3em}





\subhead{R4C13:} \textit{Section 6.4: Unclear what the "gist()" function does (might need a reference?)}

\vspace{.25em}

\subhead{Response:} ``Gist'' stands for Generalized Search Tree in PostgreSQL:\url{https://www.postgresql.org/docs/12/textsearch-indexes.html}. We have added a reference in Section \ref{subsec:datafetching}. 

\vspace{3em} 






\subhead{R4C14:} \textit{Section 7: "we build" seems like the wrong tense here, and the "etc." that appears at the end of the section isn't acceptable when listing explicit examples.}

\vspace{.25em}

\subhead{Response:} We changed ``we build'' to ``we have built'' and removed ``etc.''

\vspace{3em}

